Prompting for Multimodal Hateful Meme Classification

Hateful meme classification is a challenging multimodal task that requires complex reasoning and contextual background knowledge. Ideally, we could leverage an explicit external knowledge base to supplement contextual and cultural information in hateful memes. However, there is no known explicit external knowledge base that could provide such hate speech contextual information. To address this gap, we propose PromptHate, a simple yet effective prompt-based model that prompts pre-trained language models (PLMs) for hateful meme classification. Specifically, we construct simple prompts and provide a few in-context examples to exploit the implicit knowledge in the pre-trained RoBERTa language model for hateful meme classification. We conduct extensive experiments on two publicly available hateful and offensive meme datasets. Our experimental results show that PromptHate is able to achieve a high AUC of 90.96, outperforming state-of-the-art baselines on the hateful meme classification task. We also perform fine-grained analyses and case studies on various prompt settings and demonstrate the effectiveness of the prompts on hateful meme classification.

==> Experiment_Prev.tex <==
In this section, we first provide a brief introduction to the datasets and evaluation setting. Next, we present a set of experiments conducted to evaluate \textsf{PromptHate}'s hateful meme classification performance in supervised and few-shot setting. We also conduct studies to understand the effects of various prompt settings, and discuss the limitations of our model via error case studies. 

\subsection{Datasets}
Two publicly available datasets are used in our experiments: the \textbf{Facebook Hateful Meme} dataset (FHM)~\cite{DBLP:conf/nips/KielaFMGSRT20} and the \textbf{Harmful Meme} dataset (HarM)~\cite{DBLP:conf/acl/PramanickDMSANC21}. Table~\ref{tab:dataset} outlines the statistical distributions of the two datasets.

\textbf{Facebook Hateful Meme (FHM)}: The dataset was constructed and released by Facebook as part of a challenge to crowd-source multimodal hateful meme classification solutions. The dataset contains $10K$ memes with binary labels (i.e., hateful or non-hateful). We do not have labels of the memes in the test split. Therefore, we utilize the \textit{dev-seen} split as the \textit{test}.

\textbf{Harmful Meme (HarM)}: The dataset is constructed with real COVID-19 related memes collected from Twitter. The memes are labeled with three classes: \textit{very harmful}, \textit{partially harmful}, and \textit{harmless}. We combine the \textit{very harmful} and \textit{partially harmful memes} into hateful memes and regard harmless memes as non-hateful memes.

\begin{table}[t]
\caption{Statistical summary of FHM and HarM datasets.}
  \label{tab:dataset}
  \begin{tabular}{c|cc|cc}
    \hline
    \textbf{Datasets}& \multicolumn{2}{c|}{\textbf{Train}} & \multicolumn{2}{c}{\textbf{Test}}\\
    & \#Hate. & \#Non-hate. & \#Hate. & \#Non-hate.\\
    \hline\hline
    FHM & 3,050 & 5,450 &  250 & 250 \\
    HarM & 1,064 & 1,949 & 124 & 185\\
    \hline

\end{tabular}
\end{table}

\subsection{Evaluation Settings}
\subsubsection{Evaluation Metrics}
We adopt the evaluation metrics commonly used in existing hateful meme classification studies \cite{DBLP:conf/nips/KielaFMGSRT20,zhu2020enhance,zhou2020multimodal,DBLP:journals/corr/abs-2012-07788,DBLP:journals/corr/abs-2012-12975}: Area Under the Receiver Operating Characteristic curve (AUROC) and Accuracy (Acc).  In order to report more reliable results, we measure the average performance of models under five random seeds. All models use the same set of random seeds.

\subsubsection{Baselines}
We benchmark \textsf{PromptHate} against the state-of-the-art hateful meme classification models. Specifically, we compare with two types of baseline models: (a) \textit{classic two-stream models} and (b) \textit{multimodal pre-trained models}. Both types of models are discussed in the earlier Section~\ref{sec:related}. We select two classic two-stream baselines that utilize Faster R-CNN~\cite{ren2016faster} as the image encoder but adopt different text encoders. Namely, \textbf{MM-LSTM}, which adopts the Long-short Term Memory Networks~\cite{DBLP:journals/neco/HochreiterS97} as the text encoder, and \textbf{MM-BERT} that uses the pre-trained bidirectional encoder representations from transformers~\cite{devlin2018bert}. For both two-stream models, the multi-head attention~\cite{vaswani2017attention} is exploited for multi-modalities interaction.

Multimodal pre-trained models were also explored for hateful meme classification. For our experiments, we consider \textbf{VisualBERT}~\cite{li2019visualbert} pre-trained on the \textit{MS COCO} dataset~\cite{DBLP:conf/eccv/LinMBHPRDZ14}, and \textbf{VilBERT}~\cite{lu2019vilbert} pre-trained on the \textit{Concept Caption} dataset~\cite{DBLP:conf/acl/SoricutDSG18}. We have also included \textbf{DisMultiHate}~\cite{DBLP:conf/mm/LeeCFJC21}\footnote{We use the code published by the author and re-run the model for five-fold cross validation.}, a recent model that achieved state-of-the-art performance on the hateful meme classification task. The existing studies have also explored augmenting the models' input  with meme's entity and demographics information to improve hateful meme classification performance. Therefore, we also include variants of the \textbf{PromptHate} and baselines augmented with these information: \textbf{PromptHate-det}, \textbf{MM-BERT-det}, \textbf{VisualBERT-det}, and \textbf{VilBERT-det}. Note that \textbf{DisMultiHate} has already incorporated the entity and demographics information in its model design.

As \textsf{PromptHate} utilizes image captions to represent image information and its base model is RoBERTa~\cite{DBLP:journals/corr/abs-1907-11692}, we also create another baseline, \textbf{RoBERTa-Cap-det}, that fine-tunes a pre-trained RoBERTa with the meme's text, image caption, entity and demographics information  for hateful meme classification. 

\subsection{Comparison with Baselines}
\label{sec:experiment-results}

\begin{table}[t]
\caption{Experimental results of models on \textbf{FHM} and \textbf{HarM}.}
  \label{tab:exp-results}
  \begin{tabular}{c|cc|cc}
    \hline
    \textbf{Model}& \multicolumn{2}{c|}{\textbf{FHM}} & \multicolumn{2}{c}{\textbf{HarM}}\\
    & AUC. & Acc. & AUC. & Acc.\\
    \hline\hline
    MM-LSTM &65.92 & 56.31 &80.18&68.35 \\
    MM-BERT &68.89 &61.40 &81.57&74.56 \\
    Visual BERT &68.95 &60.00 &79.77&72.69 \\
    ViLBERT &72.57 &60.72 &83.23&75.53 \\
    \hline
    MM-BERT-det &79.71 &70.84 &84.17&77.74 \\
    Visual BERT-det &72.59 &63.12 &82.28&75.60 \\
    ViLBERT-det &75.75 &66.08 &84.90&75.47 \\
    RoBERTa-Cap-det &79.57 &69.64 & 89.94&80.26 \\
    DisMultiHate
    &79.63 &69.20 &83.77&74.69 \\
    \hline
    PromptHate &77.35 &66.96 &86.47 &75.79 \\
    PromptHate-det &\textbf{82.27} &\textbf{72.36} & \textbf{90.63}  & \textbf{82.46}\\
    \hline
\end{tabular}
\end{table}

Table~\ref{tab:exp-results} shows the hateful meme classification results of \textsf{PromptHate} and the baselines on the FHM and HarM datasets. The highest scores are highlighted in \textbf{bold}. Concurring with existing studies, the baselines augmented with demographics and entities information performed better for the hateful meme classification task. Specifically, \textsf{PromptHate-det} has achieved the best performance among the models. We noted that even without the data augmentation, \textsf{PromptHate} outperformed the two-stream baselines and multimodal pre-trained baselines on the hateful meme classification task by a large margin (over $5\%$ in terms of both AUC-ROC and accuracy on the FHM dataset). The impressive performance could be attributed to \textsf{PromptHate}'s leverage on implicit and unstructured knowledge in pre-trained RoBERTa to improve hateful meme classification. \textsf{PromptHate-det} is also observed to outperform RoBERTa-Cap-det, suggesting that prompt-tuning on PLMs would yield better performance compared to fine-tuning PLMs.

\subsection{Few-shot Classification} 

\begin{figure}[t] 
	\centering
	\setlength{\tabcolsep}{0pt} % Default value: 6pt
	\renewcommand{\arraystretch}{0} % Default value: 1
	\begin{tabular}{ccc}
		\includegraphics[scale = 0.33]{images/few-shot.pdf} 
	\end{tabular}
	\caption{The performance of \textsf{PromptHate} and baselines under few-shot learning setting. Figures in the first row are for FHM while figures in the second row for HarM.}
	\label{fig:few_shot}
\end{figure}


Prompt-based methods have shown superiority in few-shot settings for unimodal classification tasks such as sentiment classification. For our study, we extend the few-shot evaluation to our multimodal hateful meme classification task. Specifically, we perform $k$-shot few-shot learning setting where we randomly pick $k$ positive and negative training examples to train \textsf{PromptHate-det} and baselines. We report the average performance on the test split when models trained with five different and randomly sampled few-shot training set.
For more competitive comparison, we select the better performance baselines: \textbf{DisMultiHate}, \textbf{VilBERT-det}, \textbf{VisualBERT-det}, and \textbf{RoBERTa-Cap-det}. We test the few-shot capability of models with varying number of shots $k$. Considering that the nature of few-shot learning is to achieve good performance with minimum training examples, we set the maximum number of training instances to half the original training split while maintaining the size of the test splits. To the best of our knowledge, this is the first study that examines hateful meme classification in the few-shot setting.  

The few-shot learning results are presented in Figure~\ref{fig:few_shot}. We observe that when $k$ is small (i.e., less than 10\% training instances), the performance of the models is no better than random guesses, suggesting the difficulty of the hateful meme classification task. Nevertheless, we observe that using 20\% training instances, \textsf{PromptHate-det} is able to steadily outperform the baselines in the hateful meme classification task. With 30\% training instances, \textsf{PromptHate-det} is able to achieve performances that are comparative to baselines trained on full training datasets. The results demonstrated \textsf{PromptHate-det}'s ability to achieve reasonably good performance on the hateful meme classification task, even with few training instances.


\subsection{Parametric Analysis}
\textsf{PromptHate} has a number of key components that may influence its performance on the hateful meme classification task. In this section, we perform parametric analysis on two main components in \textsf{PromptHate}: (a) image-to-text caption generation, and (b) multi-query ensemble strategy. 

\subsubsection{Varying image caption} A key data-preprocessing step in \textsf{PromptHate} is to covert the image into textual captions as input for PLMs. Therefore, the quality and expressiveness of the image captions may affect on the prompting, and ultimately affect the hateful meme classification performance. To investigate this effect, we experiment with image captions generated with ClipCap~\cite{DBLP:journals/corr/abs-2111-09734} pre-trained on different datasets, namely, MS COCO~\cite{DBLP:conf/eccv/LinMBHPRDZ14,DBLP:journals/corr/ChenFLVGDZ15} and Conceptual Caption (CC)~\cite{DBLP:conf/acl/SoricutDSG18}. 

\begin{table}[t]
\caption{\textsf{PromptHate-det} performance with different image captions.}
  \label{tab:ablation-cap}
  \begin{tabular}{c|cc|cc}
    \hline
    \textbf{Model}& \multicolumn{2}{c|}{\textbf{FHM}} & \multicolumn{2}{c}{\textbf{HarM}}\\
    & AUC. & Acc. & AUC. & Acc.\\
    \hline\hline
    ClipCap+COCO &78.72&70.20& 87.25&78.38  \\ 
    ClipCap+CC &82.27 &72.36 &90.63  &82.46\\
\hline
\end{tabular}
\end{table}

Table~\ref{tab:ablation-cap} shows \textsf{PromptHate-det}'s performance with image captions generated using ClipCap pre-trained on COCO and CC. We observe that the ClipCap pre-trained on CC yields better performance than that pre-trained with COCO. A possible reason could be that the CC dataset is mainly images from web pages, which are more similar to the meme images. For instance, considering the example meme image captions generated in Table~\ref{tab:cap-comp}, we notice that ClipCap pre-trained on CC provided more detailed descriptions (e.g., the relation of the man and the woman of the first meme and the characteristic of the sign in the second meme) compared to COCO. The difference in their performance is also significant, suggesting the importance of good quality captions in applying prompt-based models for hateful meme classification.   


\begin{table}[t]
  \centering
  \caption{Example meme image captions generated.}
  \label{tab:cap-comp}
  \begin{tabular}{|c|p{2.6cm}|p{2.6cm}| }
    \hline
    \textbf{Meme} & \begin{minipage}[b]{0.32\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{comparison/kitchen.png}}
	\end{minipage} &
    \begin{minipage}[b]{0.32\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{comparison/warning.png}}
	\end{minipage}
	\\ \hline
    \textbf{ClipCap+COCO} &a man and a woman are in a kitchen.
    &a sign that is on the side of a hill.
	\\\hline
    \textbf{ClipCap+CC} &young couple in love looking at each other in kitchen.
    &warning sign at the entrance to the quarry. 
    \\ \hline
    \end{tabular}
\end{table}


\begin{table}[t]
\caption{\textsf{PromptHate-det} performance when varying $m$.}
  \label{tab:ablation-query}
  \begin{tabular}{c|cc|cc}
    \toprule
    \textbf{Setting}& \multicolumn{2}{c|}{\textbf{FHM}} & \multicolumn{2}{c}{\textbf{HarM}}\\
    & AUC. & Acc. & AUC. & Acc.\\
    \midrule
    m=1  &81.91 &71.56 &89.64&82.40 \\ 
    m=2  &\textbf{82.27} &72.36 &\textbf{90.63}&\textbf{82.46} \\ 
    m=3  &81.87 &\textbf{72.60} &89.69 &80.52 \\ 
    m=4  &82.00 &71.64 &89.78 &82.01 \\ 
    m=5  &81.87 &72.60 &90.57 &79.61 \\ 
    \bottomrule
\hline
\end{tabular}
\end{table}

\subsubsection{Varying Multi-Query Ensemble} 
In Section \ref{sec:ensemble}, we discuss a multi-query ensemble strategy adopted by \textsf{PromptHate-det} to predict the inference instance using  multiple pairs of demonstrations. To examine the impact of the multi-query ensemble strategy on \textsf{PromptHate-det}'s performance, we vary the $m$ pairs of demonstrations used. Table~\ref{tab:ablation-query} shows the results on FHM and HarM datasets. Interestingly, we observe that increasing the number of demonstration pairs (i.e., $m$) did not enhance the performance significantly. A possible reason may be that the sampled demonstration may be too diverse. For instance, the sampled positive and negative demonstrations may target protected characteristics different from the inference instance. Nevertheless, we noted that increasing $m$ will take up more time for inference. Thus, considering the trade-off between the performance and inference time, we select $m=2$ as the multi-query ensemble settings for both datasets. For future works, we will explore other strategies for selecting better demonstrations for \textsf{PromptHate}.  
 
\subsection{Prompt Engineering} 
Designing good prompts is essential to prompt-based models. In this section, we discuss how the varying of prompts will affect \textsf{PromptHate}'s performance in hateful meme classification. 

\subsubsection{Engineering Label Words}
The label words are individual words representing the labels used in prompt generation. We investigate the effects of replacing the prompts in \textsf{PromptHate-det} with different sets of labels words. Specifically, we replace the labels words in the prompt's positive and negative demonstrations in our experiments. For example, in the first row in Table~\ref{tab:verbalizer}, we use ``\textit{It was \textbf{normal}}'' for positive demonstrations (i.e., non-hateful memes), and ``\textit{It was \textbf{hate}}'' for negative demonstration (i.e., hateful memes). Conversely, in the second row, we swap the label words and use `\textit{It was \textbf{hate}}'' for positive demonstrations (i.e., non-hateful memes), and  ``\textit{It was \textbf{normal}}'' for negative demonstration (i.e., hateful memes). The intuition for the experimental design is that we aim to examine how the label word's semantic affects hateful meme classification memes. For instance, will assigning a positive word (e.g., normal) to be the label word for negative demonstrations (i.e., hateful memes) hamper the \textsf{PromptHate-det}'s performance? We have also conducted the experiments on full training instances and few-shot setting, i.e., using only 10\% of training instances. 

Table~\ref{tab:verbalizer} shows the results of our label words experiments. We notice that, in most cases, models with the label words with aligned semantic class performed better. For instance, when using \textit{good} representing the positive demonstrations (i.e., non-hateful memes) and \textit{bad} for the negative demonstration (i.e., hateful memes) is better than using the reversed mapping. More interestingly, we notice that the difference between the performance of label words with aligned semantic class and reversed mapping is more significant in few-shot setting than full training instances. A possible reason could be in the few-shot setting, the \textsf{PromptHate-det} will rely more on the label words' semantics to extract implicit knowledge for hateful meme classification. Thus, the label words with aligned semantic class will provide better context in the prompt to improve hateful meme classification when there are insufficient observations in training instances. Conversely, when \textsf{PromptHate-det} is trained with enough instances, the representations of the label words are updated to be closer to the hateful meme classification task.      


\begin{table}[t]
\caption{\textsf{PromptHate-det} performance  with various label words.}
  \label{tab:verbalizer}
  \begin{tabular}{c|cc|cc|cc}
    \hline
    \multirow{2}{*}{\textbf{Setting}} &
    \multicolumn{2}{c|}{\textbf{Label Words}}& \multicolumn{2}{c|}{\textbf{FHM}} & \multicolumn{2}{c}{\textbf{HarM}}\\

    & Pos. & Neg. & AUC. & Acc. & AUC. & Acc.\\
    \hline\hline
    \multirow{6}{*}{Full} & Normal & Hate & 82.15 & 72.16 &89.51&79.94 \\
    & Hate & Normal &81.16 &70.96 &88.91&79.22 \\
    &Benign & Offensive &82.90 &72.60 &88.88&80.58 \\
    &Offensive & Benign &81.24 &71.00 &88.95&80.26 \\ 

    &Good & Bad &82.27 &72.36 &90.63&82.46 \\
    &Bad & Good &81.20 &71.64 &89.60&80.19 \\ 
    \hline\hline
    \multirow{6}{*}{Few-Shot} & Normal & Hate &69.21 &63.88&86.45&72.69 \\
    &Hate & Normal &62.17 &57.56&84.79&72.04 \\
    &Benign & Offensive &68.91 &63.68&83.29&62.91 \\
    &Offensive & Benign &64.80 &59.44&79.20&61.75 \\ 
    &Good & Bad & 69.30&63.76&84.78&74.63 \\
    &Bad & Good &67.40 &61.64&83.68&68.03 \\ 
\hline
\end{tabular}
\end{table}

\subsubsection{Prompt with Hateful Target Information}
Existing studies have found that modelling target information (i.g., the victim of the hateful content) can help improve hateful meme classification~\cite{DBLP:conf/mm/LeeCFJC21}. In this study, we explore the effect of explicitly including the target information in prompts.

The FHM and HarM datasets are annotated with target information. For instance, FHM hateful memes are annotated with five target categories: \textit{race}, \textit{disability}, \textit{nationality}, \textit{sex} and \textit{religion}. Hateful memes on HarM are annotated with four target categories: \textit{society}, \textit{individual}, \textit{community} and \textit{organization}. For our experimental design, we change the prompt template: from ``\textit{It was \textbf{[MASK]}.}'' to ``\textit{It was \textbf{[LABEL\_MASK]} targeting at \textbf{[TARGET\_MASK]}.}''. For example, if it is a hateful meme targeting nationality, the template will be ``\textit{It was \textbf{bad} targeting at \textbf{nationality}}.'' If the meme is non-hateful, the \textbf{[TARGET\_MASK]} will be replaced with \textbf{nobody}. During model training, we model the loss from prediction of \textbf{[LABEL\_MASK]} in the inference instance, and the masked word for labels and targets will be provided in demonstrations. Similar to our earlier experiments, we perform the target augmentation experiments on full training instances and few-shot setting. 

Table~\ref{tab:targets} shows the results of the \textsf{PromptHate-det} performance with and without target information. In the full training instance setting, we observe marginal differences in performance after modelling target information in prompts. More interestingly, in the few-shot setting, we observe modelling target information in prompts worsens \textsf{PromptHate-det} hateful meme classification performance. A possible reason may be that learning to extract targets in memes adds auxiliary burden to the model. We will explore other strategies to better utilize target information in the prompt-based model for hateful meme classification for future works.

\begin{table}[t]
\caption{\textsf{PromptHate-det} performance with and without target.}
  \label{tab:targets}
  \begin{tabular}{c|c|cc|cc}
    \hline
    \multirow{2}{*}{\textbf{Setting}} &\textbf{Model}& \multicolumn{2}{c|}{\textbf{FHM}} & \multicolumn{2}{c}{\textbf{HarM}}\\
   & & AUC. & Acc. & AUC. & Acc.\\
    \hline\hline
   \multirow{2}{*}{Full}& w/o Target &82.27  &72.36 &90.63 &82.46\\
    & w Target & 82.08&72.28 &88.62 &80.00 \\
    \hline
    \multirow{2}{*}{Few-Shot} & w/o Target &69.30&63.76&83.95&73.53\\
    & w Target &62.76&56.28&70.44&60.58\\
\hline
\end{tabular}
\end{table}

To further investigate the issues with incorporating target information in prompts, we sampled some memes from the FHM dataset and visualized \textsf{PromptHate-det}'s prediction results in Table~\ref{tab:comp-vis}. The incorrect predictions are labelled in red. We have also visualized distributions of the predicted target in the given meme (i.e., \textbf{[TARGET\_MASK]}). From Table~\ref{tab:comp-vis}, we notice that the \textsf{PromptHate-det} with target information is able to correctly predict the targets in the hateful meme even when it incorrectly classifies the memes (e.g., the right two memes). Specifically, for the first meme on the left, the model correctly predicted that it was targeting race when there was no mention of the race in the meme. Therefore, the target distributions could help improve the \textsf{PromptHate-det}'s interpretability. Nevertheless, the incorrect class label prediction also highlights the difficulty of hateful meme classification as the task may require more than target comprehension to achieve good performance.

\begin{table*}[h]
  \centering
  \caption{Example predictions of \textsf{PromptHate-det} with and without target information.}
  \label{tab:comp-vis}
  \begin{tabular}{|c|c|c|c|c| }
    \hline
    \textbf{Meme} & \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{comparison/comp-3k-img.pdf}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{comparison/comp-woman-img.pdf}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{comparison/comp-wrong-religion-img.pdf}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{comparison/comp-wrong-obama-img.pdf}}
	\end{minipage}\\
    \hline
    \textbf{Target Distributions} & \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{comparison/comp-3k-chart.png}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{comparison/comp-woman-chart.png}}
	\end{minipage} &
   \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{comparison/comp-wrong-mosque-chart.png}}
	\end{minipage} &
    \begin{minipage}[b]{0.38\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{comparison/comp-wrong-pbama-chart.png}}
	\end{minipage}
   \\\hline
	\textbf{w Target.}  &Hateful & Hateful &\color{red}Non-Hateful  & \color{red} Hateful \\
	\hline
	\textbf{w/o Target} &\color{red} Non-hateful & \color{red} Non-hateful&  Hateful& Non-hateful \\
	\hline
	\textbf{Ground Truth}  & Hateful & Hateful & Hateful & Non-Hateful \\
	\hline 
    \end{tabular}
\end{table*}

\subsection{Error Analysis}
Besides analyzing \textsf{PromptHate} quantitatively performance over the state-of-the-art baselines, we are also interested in examining the classification errors of \textsf{PromptHate}. Table~\ref{tab:error} illustrates four selected examples of \textsf{PromptHate}'s wrongly classified memes. For example, \textsf{PromptHate} has classified the first meme to be non-hateful when the actual label of the meme is hateful. 

From the examples, we notice that the captions generally describe the contents of images. However, it may ignore some essential attributes for hateful meme detection. For instance, the captions are unable to capture important information such as ``\textit{Jesus}'' in the first meme or ``\textit{Jihadism}'' in the second meme. This missing information is supplemented by the augmented entity and demographic information, which aligns with our quantitative findings that entity and demographic augmentation improve hateful meme classification. Nevertheless, we also observed that even after augmented with additional descriptions for the images, \textsf{PromptHate} still makes incorrect predictions for the memes in Table~\ref{tab:error}. There could be multiple reasons for the incorrect predictions. Firstly, it could be that the presented information is still inadequate to provide enough context to make a correct prediction. For instance, in the third meme, the ``biting'' or ``eating'' action is missing from the captions and the addition image description. Thus, \textsf{PromptHate} is not able to retrieve the context that the meme is ridiculing Asians' ``dog-eating'' behaviour, and it is hateful. Secondly, there could be some biases learned by the model. For instance, in the last meme, \textsf{PromptHate} may predict the meme to be hateful because of the rainbow flag, which is an icon for the LGBT community, and there are other memes that attacked the LGBT community using memes with the iconic rainbow flag. Lastly, some form of advanced reasoning would be required to understand the hateful context presented in this meme. For instance, in the first meme, \textsf{PromptHate} is unable to reason that the meme is equating Jesus on the cross as a scarecrow as it is not a common slur that is found in other memes. The limitations of \textsf{PromptHate} also suggested areas of improvement that require deeper research in future works. 


\begin{table*}[h]
  \centering
  \caption{Error analysis of wrongly predicted memes.}
  \label{tab:error}
  \begin{tabular}{|c|p{3.2cm}|p{3.2cm}|p{3.2cm}|p{3.2cm}| }
    \hline
    \textbf{Meme} & \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{error/error-scarecrow.pdf}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{error/error-terror.pdf}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{error/error-dot.pdf}}
	\end{minipage} &
    \begin{minipage}[b]{0.35\columnwidth}
		\centering
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{error/error-rainbow.pdf}}
	\end{minipage}\\\hline
    \textbf{Ground Truth} & Hateful & Hateful & Hateful & Non-Hateful\\\hline
    \textbf{Prediction} & \color{red} Non-hateful & \color{red} 
    Non-hateful & \color{red} Non-hateful & \color{red} Hateful\\\hline
    \textbf{Meme text} &the original scarecrow &welcome to melbourne &when you date an asian boy and you trynna get his family to accept you&you either die a hero, or live long enough to become the villain\\\hline
    \textbf{Captions} &builder crucified on the cross
    &soldiers stand in front of a building &
    portrait of a young woman with her pet dog& 
    a man dressed as a rainbow holding a  flag and dancing in the crowd\\ \hline
    \textbf{Entity} & Crucifix Life, Resurrection of Jesus, Spiritual death, Kirkmont Presbyterian Church Salvation, jesus died in the cross& Jihadism, United Nations Editorial Jihadism& None&Rainbow flag, Flag bisexual, Transgender flags, Bisexuality \\\hline
    \textbf{Demographics} &None & None &Black female & Latino Hispanic Male\\\hline
    \end{tabular}
\end{table*}


